Context in Informational Bias Detection

Informational bias is bias conveyed through sentences or clauses that provide tangential, speculative or background information that can sway readers' opinions towards entities. By nature, informational bias is context-dependent, but previous work on informational bias detection has not explored the role of context beyond the sentence. In this paper, we explore four kinds of context for informational bias in English news articles: neighboring sentences, the full article, articles on the same event from other news publishers, and articles from the same domain (but potentially different events). We find that integrating event context improves classification performance over a very strong baseline. In addition, we perform the first error analysis of models on this task. We find that the best-performing context-inclusive model outperforms the baseline on longer sentences, and sentences from politically centrist articles.

==> sections/discussion.tex <==
The influence of news source origin on model performance suggests categorical differences in the way newspapers source use background information to influence opinion.
Future work could explore how bias in Fox News articles differs from bias in other sources, and whether these differences are large enough that domain-adaptation to specific sources boosts performance compared to classifying news sources together.
Additionally, future dataset may need to ensure a balance of sources that represent different layers and sections of society.
Future work could also extend context-inclusion experiments to token classification.

